LeCaRDv2: A Large-Scale Chinese Legal Case Retrieval Dataset

As an important component of intelligent legal systems, legal case retrieval plays a critical role in ensuring judicial justice and fairness. However, the development of legal case retrieval technologies in the Chinese legal system is restricted by three problems in existing datasets: limited data size, narrow definitions of legal relevance, and naive candidate pooling strategies used in data sampling. To alleviate these issues, we introduce LeCaRDv2, a large-scale Legal Case Retrieval Dataset (version 2). It consists of 800 queries and 55,192 candidates extracted from 4.3 million criminal case documents. To the best of our knowledge, LeCaRDv2 is one of the largest Chinese legal case retrieval datasets, providing extensive coverage of criminal charges. Additionally, we enrich the existing relevance criteria by considering three key aspects: characterization, penalty, procedure. This comprehensive criteria enriches the dataset and may provides a more holistic perspective. Furthermore, we propose a two-level candidate set pooling strategy that effectively identify potential candidates for each query case. It's important to note that all cases in the dataset have been annotated by multiple legal experts specializing in criminal law. Their expertise ensures the accuracy and reliability of the annotations. We evaluate several state-of-the-art retrieval models at LeCaRDv2, demonstrating that there is still significant room for improvement in legal case retrieval. The details of LeCaRDv2 can be found at the anonymous website https://github.com/anonymous1113243/LeCaRDv2.

==> brain_signals_decoding.tex <==
\subsection{Brain Signals Decoding}

Existing works in multichannel \ac{EEG}-based prediction usually need effective feature extraction. 
Several features are proposed throughout literature and among these features, \ac{DE} is widely used and performs better than other features including band power, rational asymmetry, and differential asymmetry in an multi-channel \ac{EEG}-based emotion recognition task~\cite{duan2013differential}.
% 需要前面介绍一下我们做实验的环境，之前讨论的时候忘记加这章了
Therefore, we extract \ac{DE} features using Short Time Fourier Transform over five frequency bands~(delta: 0.5-4Hz, theta: 4-8Hz, alpha: 8-13Hz, beta: 14-30Hz, gamma: 30-50Hz) in 62 distinct \ac{EEG} channels except for two re-reference channels.
For classification model, we apply \ac{GBDT}, which can automatically choose and combine the \ac{EEG} features and it has shown effective in usefulness estimation with multichannel \ac{EEG} features~\cite{2109.10560}.
To train the prediction model, we use the Search-Brainwave dataset~\footnote{http://www.thuir.cn/group/YQLiu/datasets/SearchBrainwaveDataset.zip}.
The dataset contains \ac{EEG} data recorded during the 18 participants doing pre-defined search tasks in a period of 60 minutes as well as the usefulness annotation for each search result.
To tune the hyper parameters, including learning rate, estimator number, leaf nodes, and the maximum tree depth, we applied the protocol of leave-one-participant-out.
The protocol means that we apply data of each participant for validation and train the classifier with left participants.
The parameters are tuned according to the averaged validation \ac{AUC} of each participant and then we train our final classifier with all data.
As a result, the system can achieve an averaged \ac{AUC} of 0.69 in validation and the whole steps~(feature extraction and \ac{GBDT}-based classification) described above cost averagely 0.2 seconds in our practice.

Now that we can predict the satisfaction feedback and understand the perceived usefulness of the search results, our search system can automatically adjust to improve the search process.
In our practice, we apply a simple strategy as a first step to utilize brain signals as feedback for a more proactive search system.
Before our experiment, each search result involved has been annotated with some subtopics by topic model. 
On the one hand, when the system notice that the user perceive certain landing page is useful, search results share similar subtopics would be moved to the top.
On the other hand, when we detect that the user is unsatisfied with certain landing page, we will re-rank the search result list and the results share the same subtopics will be moved to the back.
The certain landing page refers to the top-ranked page as described in Section~\ref{SYSTEM OVERVIEW}.
Note that we focus on the effectiveness of brain signals can be decoded as feedback for a better search performance in a real-time system, the methods of how to combine these feedback with other evaluation framework are left as future work.
% Satisfaction Prediction 
% Search Results Re-ranking

==> de.tex <==
% !TEX root = ./sample-sigconf.tex 
\usepackage{acronym}

\acrodef{IR}{Information Retrieval}
\acrodef{MLP}{multilayer perceptron}
\acrodef{SERP}{Search Engine Result Page}
\acrodef{ERP}{Event Related Potential}
\acrodef{EEG}{electroencephalogram}
\acrodef{GBDT}{Gradient Boosting Decision Tree}
\acrodef{SST}{SST-EmotionNet}
\acrodef{AUC}{Area Under Curve}
\acrodef{IN}{Information Need}
\acrodef{fMRI}{functional Magnetic Resonance Imaging}
\acrodef{BMI}{Brain–Machine Interface}
\acrodef{BP}{Band Power}
\acrodef{DE}{differential entropy}
\acrodef{RASM}{rational asymmetry}
\acrodef{DASM}{differential asymmetry}
\acrodef{SVM}{Support Vector Machines}
\acrodef{DBN}{Deep Belief Networks}
\acrodef{KNN}{k-Nearest Neighbors}
\acrodef{HBG}{Height-Biased Gain}

\acrodef{BMSI}{Brain Machine Search Interface}
\acrodef{SSVEP}{Steady-State Visually Evoked Potential}
\acrodef{CCA}{Canonical Correlation Analysis}
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\newcommand{\todo}[1]{\textcolor{red}{\textbf{[#1]}}}


